Clustering-Based Balanced Sampling and Allocation with Data Parallelism for High-Performance Fine-Tuning

Instruction-tuning datasets for large language models (LLMs) are often large, redundant, and imbalanced, limiting efficient adaptation. Naive large-batch fine-tuning repeatedly includes overrepresented sample groups while weakly covering underrepresented but informative ones, especially under data parallelism (DP) across multiple GPUs. We propose CluSTER, a Cluster-aware balanced Sampling framework for Training Efficient data Reduction in DP instruction tuning. CluSTER curates a representative reduced dataset through gradient-space clustering and DP-aware balanced allocation, ensuring dual-level coverage across clusters and workers, while preserving the original data distribution by weighted update. As a result, CluSTER reduces redundant computation and improves training stability without compromising model quality. Across multiple instruction-tuning datasets, CluSTER reduces training time by up to 69.6% with almost no accuracy loss compared to prior sampling and data reduction methods. Code is available at https://github.com/kaist-dmlab/CluSTER.

==> table_efficiency.tex <==
\centering
\caption{Comparison of training efficiency and average performance relative to the full dataset fine-tuning baseline. $\Delta$ Score is computed as the difference in average score with respect to the full dataset random sampling baseline.}
\label{tab:training_time_perf}
\begin{minipage}{0.49\textwidth}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{Data Ratio} & \textbf{Time (h)} & \textbf{Reduction (\%)} & \textbf{Score} & \textbf{$\Delta$ Score (\%)} \\
\midrule
\multicolumn{6}{c}{\textbf{CodeLlama-Python-7B} fine-tuned on \textbf{Evol-Instruct-Code-80K}} \\
\midrule
Full & 100\% & 0.82 & -- & 52.1 & -- \\
\midrule
\multirow{3}{*}{Random}
    & 68\% & 0.56 & 31.2\% ↓ & 42.5 & $-18.4$ \\
    & 51\% & 0.44 & 45.8\% ↓ & 42.6 & $-18.2$ \\
    & 35\% & 0.28 & 65.7\% ↓ & 41.4 & $-20.5$ \\
\midrule
\multirow{3}{*}{\algname{}}
    & 68\% & 0.76 & 7.3\% ↓ & 52.3 & $+0.3$ \\
    & 51\% & 0.62 & 24.4\% ↓ & 51.8 & $-0.6$ \\
    & 35\% & 0.48 & 41.5\% ↓ & 49.9 & $-4.2$ \\
\bottomrule
\end{tabular}}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{Data Ratio} & \textbf{Time (h)} & \textbf{Reduction (\%)} & \textbf{Score} & \textbf{$\Delta$ Score (\%)} \\
\midrule
\multicolumn{6}{c}{\textcolor{red}{\textbf{TBD} fine-tuned on \textbf{TBD}}} \\
\midrule
Full & 100\% & 0.82 & -- & 52.1 & -- \\
\midrule
\multirow{3}{*}{Random}
    & 68\% & 0.56 & 31.2\% ↓ & 42.5 & $-18.4$ \\
    & 51\% & 0.44 & 45.8\% ↓ & 42.6 & $-18.2$ \\
    & 35\% & 0.28 & 65.7\% ↓ & 41.4 & $-20.5$ \\
\midrule
\multirow{3}{*}{\algname{}}
    & 68\% & 0.76 & 7.3\% ↓ & 52.3 & $+0.3$ \\
    & 51\% & 0.62 & 24.4\% ↓ & 51.8 & $-0.6$ \\
    & 35\% & 0.48 & 41.5\% ↓ & 49.9 & $-4.2$ \\
\bottomrule
\end{tabular}}

==> table_magi_old.tex <==
\begin{table*}[!t]
\centering
\caption{
Pass@1\,(\%) and training time for different data sampling strategies on \textrm{CodeLlama-7B} fine-tuned with \textrm{Magicoder-OSS-Instruct-75K}.
Cluster balancing keeps 79\% of the original dataset; applying intra-cluster selection ratios $r \in \{1.00, 0.75, 0.50\}$ results in effective data uses of 79\%, 59\%, and 40\% of the original dataset, respectively.
% Pass@1 is evaluated with greedy decoding.
% $\Delta$ Score indicates the performance gap relative to the full-data baseline.
\textbf{Bold} indicates the best score at each data usage.
\colorbox{black!10}{Gray} cells indicate reference values for comparison. 
% performance and training-time 
}
\label{tab:main_magi}
\resizebox{\linewidth}{!}{
\begin{tabular}{ll cccc cc}
\toprule
\multicolumn{2}{c}{Data Selection} & \multicolumn{4}{c}{Evaluation Benchmark} & \multicolumn{2}{c}{Training Efficiency} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-8}
\textbf{Selection Ratio} & \textbf{Sampling} & \textbf{HumanEval(+)} & \textbf{MBPP(+)} & \textbf{Average} & \textbf{$\Delta$ Score (\%)} & \textbf{Time (hr)} & \textbf{Reduction (\%)} \\
\midrule
\multirow{2}{*}{\makecell[l]{Full Dataset\\(100\%)}} 
  & Random  & 57.1{\scriptsize $\pm$ 1.5} (52.4{\scriptsize $\pm$ 2.7}) & 66.1{\scriptsize $\pm$ 0.6} (54.8{\scriptsize $\pm$ 0.6}) & \cellcolor{black!10} 57.6 & - & \cellcolor{black!10} 1.13 & - \\
  & Uniform & 54.1{\scriptsize $\pm$ 2.2} (50.0{\scriptsize $\pm$ 2.4}) & 65.0{\scriptsize $\pm$ 1.3} (54.3{\scriptsize $\pm$ 1.5}) & 55.8 & -3.08 & 1.29 & -14.5 \\
\midrule
\multirow{5}{*}{\makecell[l]{1.00\\(79.3\%)}} %No redundancy
  & Random  & \textbf{54.9{\scriptsize $\pm$ 1.6}} (49.4{\scriptsize $\pm$ 1.8}) & 65.9{\scriptsize $\pm$ 1.1} (54.7{\scriptsize $\pm$ 0.9}) & 56.2 & -2.43 & 0.90 & 20.1 \\
  & Uniform & 53.3{\scriptsize $\pm$ 2.3} (49.0{\scriptsize $\pm$ 1.7}) & 65.1{\scriptsize $\pm$ 0.3} (54.2{\scriptsize $\pm$ 0.7}) & 55.4 & -3.85 & 1.04 & 7.5 \\
  & IFD     & 53.8{\scriptsize $\pm$ 3.1} (49.8{\scriptsize $\pm$ 3.1}) & 65.3{\scriptsize $\pm$ 0.4} (54.0{\scriptsize $\pm$ 1.4}) & 55.7 & -3.29 & 0.87 & 22.6 \\
  & LESS    & 53.9{\scriptsize $\pm$ 2.2} (\textbf{50.0{\scriptsize $\pm$ 1.8}}) & 65.8{\scriptsize $\pm$ 0.2} (53.6{\scriptsize $\pm$ 0.7}) & 55.8 & -3.09 & 0.90 & 20.1 \\
  & \textbf{\algname{}} 
             & \textbf{54.9{\scriptsize $\pm$ 1.2}} (49.8{\scriptsize $\pm$ 1.5}) 
             & \textbf{67.0{\scriptsize $\pm$ 1.3}} (\textbf{55.6{\scriptsize $\pm$ 1.1}}) 
             & \textbf{56.8} & \textbf{-1.33} & 0.92 & 16.9 \\
\midrule
\multirow{5}{*}{\makecell[l]{0.75\\(59.4\%)}} 
  & Random  & 51.4{\scriptsize $\pm$ 0.7} (46.8{\scriptsize $\pm$ 1.0}) & \textbf{67.2{\scriptsize $\pm$ 1.1}} (55.1{\scriptsize $\pm$ 0.7}) & 55.1 & -4.33 & 0.67 & 40.5 \\
  & Uniform & 52.6{\scriptsize $\pm$ 2.5} (48.0{\scriptsize $\pm$ 2.9}) & 66.1{\scriptsize $\pm$ 1.2} (54.4{\scriptsize $\pm$ 1.0}) & 55.3 & -4.04 & 0.77 & 31.2 \\
  & IFD     & 50.2{\scriptsize $\pm$ 0.7} (43.9{\scriptsize $\pm$ 2.1}) & 66.3{\scriptsize $\pm$ 0.4} (54.4{\scriptsize $\pm$ 0.4}) & 53.7 & -6.76 & 0.66 & 41.6 \\
  & LESS    & 53.3{\scriptsize $\pm$ 1.8} (49.0{\scriptsize $\pm$ 1.7}) & 65.4{\scriptsize $\pm$ 1.2} (53.8{\scriptsize $\pm$ 0.4}) & 55.4 & -3.92 & 0.67 & 40.5 \\
  & \textbf{\algname{}} 
             & \textbf{54.5{\scriptsize $\pm$ 0.9} (49.4{\scriptsize $\pm$ 1.0})} 
             & 66.9{\scriptsize $\pm$ 0.5} (\textbf{55.3{\scriptsize $\pm$ 0.3}}) 
             & \textbf{56.5} & \textbf{-1.87} & 0.69 & 37.2 \\
\midrule
\multirow{5}{*}{\makecell[l]{0.50\\(39.6\%)}} 
  & Random  & 52.2{\scriptsize $\pm$ 1.3} (45.9{\scriptsize $\pm$ 1.0}) & 66.0{\scriptsize $\pm$ 0.8} (54.7{\scriptsize $\pm$ 0.9}) & 54.7 & -4.99 & 0.45 & 60.0 \\
  & Uniform & 51.8{\scriptsize $\pm$ 2.7} (46.7{\scriptsize $\pm$ 2.3}) & 64.9{\scriptsize $\pm$ 1.7} (53.7{\scriptsize $\pm$ 1.1}) & 54.3 & -5.76 & 0.53 & 52.8 \\
  & IFD     & 50.6{\scriptsize $\pm$ 0.0} (44.7{\scriptsize $\pm$ 0.3}) & 64.5{\scriptsize $\pm$ 1.2} (53.8{\scriptsize $\pm$ 1.0}) & 53.4 & -7.31 & 0.44 & 61.0 \\
  & LESS    & 53.7{\scriptsize $\pm$ 1.1} (48.2{\scriptsize $\pm$ 1.2}) &\textbf{ 66.2{\scriptsize $\pm$ 1.2}} (54.6{\scriptsize $\pm$ 2.2}) & 55.7 & -3.36 & 0.45 & 60.0 \\
  & \textbf{\algname{}} 
             & \textbf{54.0{\scriptsize $\pm$ 1.8} (49.0{\scriptsize $\pm$ 2.5})} 
             & 65.8{\scriptsize $\pm$ 1.1} (\textbf{55.0{\scriptsize $\pm$ 0.9}}) 
             & \textbf{55.9} & \textbf{-2.89} & 0.47 & 57.9 \\
\bottomrule
\end{tabular}}
\vspace{-0.1cm}
\end{table*}

==> table_main_table.tex <==
% \begin{table*}[t]
% \centering
% \caption{Performance of different data sampling strategies for \textit{CodeLlama-7B} fine-tuned on \textit{Evol-Instruct-Code-80K}. 
% The 51\% and 35\% settings correspond to 75\% and 50\% subsamples of the 68\% pruned dataset, respectively.
% Scores are pass@1 on code generation benchmarks evaluated through greedy decoding.
% For each benchmark, results are reported as score corresponding to the base and extended evaluation sets.
% \textbf{Bold} indicates the best performance within each data-ratio setting, and \underline{underline} marks the best overall score across all configurations.}
% \label{tab:main_table}
% \begin{tabular}{l l c c c}
% \toprule
% \textbf{Data Ratio} & \textbf{Sampling} & \textbf{HumanEval(+)} & \textbf{MBPP(+)} & \textbf{Average} \\
% \midrule
% \multirow{2}{*}{100\%} 
%   & Random  & 48.6(41.9) & \underline{64.5(53.3)} & 52.1 \\
%   & Uniform & 43.3(37.4) & 33.0(28.1) & 35.5 \\
% \midrule
% \multirow{4}{*}{\makecell[l]{68\%\\($r = 1.00$)}} %No redundancy
%   & Random  & 46.7(39.2) & 45.7(38.4) & 42.5 \\
%   & Uniform & 42.9(36.6) & 39.8(33.2) & 38.1 \\
%   & IFD     & 47.0(40.3) & 33.9(27.9) & 37.2 \\
%   & \textbf{\algname{}} 
%              & \underline{\textbf{50.2(44.6)}} 
%              & \textbf{62.5(52.1)} 
%              & \underline{\textbf{52.3}} \\
% \midrule
% \multirow{4}{*}{\makecell[l]{51\%\\($r = 0.75$)}} 
%   & Random  & 45.3(39.2) & 47.7(39.0) & 42.6 \\
%   & Uniform & 35.4(31.5) & 40.6(33.4) & 35.2 \\
%   & IFD     & 45.1(38.6) & 34.5(28.9) & 36.8 \\
%   & \textbf{\algname{}} 
%              & \textbf{48.5(43.5)} 
%              & \textbf{62.7(52.7)} 
%              & \textbf{51.8} \\
% \midrule
% \multirow{4}{*}{\makecell[l]{35\%\\($r = 0.50$)}} 
%   & Random  & 45.6(39.2) & 43.7(36.9) & 41.4 \\
%   & Uniform & 29.7(25.8) & 39.4(32.7) & 31.9 \\
%   & IFD     & 45.5(39.2) & 33.3(27.8) & 36.5 \\
%   & \textbf{\algname{}} 
%              & \textbf{46.4(41.7)} 
%              & \textbf{61.1(50.6)} 
%              & \textbf{49.9} \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\centering
\caption{Performance of different data sampling strategies for \textit{CodeLlama-7B} fine-tuned on \textit{Evol-Instruct-Code-80K}. 
The 51\% and 35\% settings correspond to 75\% and 50\% subsamples of the 68\% pruned dataset, respectively.
Scores are pass@1 on code generation benchmarks evaluated through greedy decoding.
For each benchmark, results are reported as score corresponding to the base and extended evaluation sets.
\textbf{Bold} indicates the best performance within each data-ratio setting, and \underline{underline} marks the best overall score across all configurations.}
\label{tab:main_table}

\begin{minipage}{0.49\textwidth}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l l c c c}
\toprule
\textbf{Data Ratio} & \textbf{Sampling} & \textbf{HumanEval(+)} & \textbf{MBPP(+)} & \textbf{Average} \\
\midrule
\multicolumn{5}{c}{\textbf{CodeLlama-Python-7B} fine-tuned on \textbf{Evol-Instruct-Code-80K}} \\
\midrule
\multirow{2}{*}{100\%} 
  & Random  & 48.6(41.9) & \underline{64.5(53.3)} & 52.1 \\
  & Uniform & 43.3(37.4) & 33.0(28.1) & 35.5 \\
\midrule
\multirow{4}{*}{\makecell[l]{68\%\\($r = 1.00$)}} %No redundancy
  & Random  & 46.7(39.2) & 45.7(38.4) & 42.5 \\
  & Uniform & 42.9(36.6) & 39.8(33.2) & 38.1 \\
  & IFD     & 47.0(40.3) & 33.9(27.9) & 37.2 \\
  & \textbf{\algname{}} 
             & \underline{\textbf{50.2(44.6)}} 
             & \textbf{62.5(52.1)} 
             & \underline{\textbf{52.3}} \\
\midrule
\multirow{4}{*}{\makecell[l]{51\%\\($r = 0.75$)}} 
  & Random  & 45.3(39.2) & 47.7(39.0) & 42.6 \\
  & Uniform & 35.4(31.5) & 40.6(33.4) & 35.2 \\
  & IFD     & 45.1(38.6) & 34.5(28.9) & 36.8 \\
  & \textbf{\algname{}} 
             & \textbf{48.5(43.5)} 
             & \textbf{62.7(52.7)} 
             & \textbf{51.8} \\
\midrule
\multirow{4}{*}{\makecell[l]{35\%\\($r = 0.50$)}} 
  & Random  & 45.6(39.2) & 43.7(36.9) & 41.4 \\
  & Uniform & 29.7(25.8) & 39.4(32.7) & 31.9 \\
  & IFD     & 45.5(39.2) & 33.3(27.8) & 36.5 \\
  & \textbf{\algname{}} 
             & \textbf{46.4(41.7)} 
             & \textbf{61.1(50.6)} 
             & \textbf{49.9} \\
\bottomrule
\end{tabular}}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l l c c c}
\toprule
\textbf{Data Ratio} & \textbf{Sampling} & \textbf{HumanEval(+)} & \textbf{MBPP(+)} & \textbf{Average} \\
\midrule
\multicolumn{5}{c}{\textcolor{red}{\textbf{TBD} fine-tuned on \textbf{TBD}}} \\
\midrule
\multirow{2}{*}{100\%} 
  & Random  & 48.6(41.9) & \underline{64.5(53.3)} & 52.1 \\
  & Uniform & 43.3(37.4) & 33.0(28.1) & 35.5 \\
\midrule
\multirow{4}{*}{\makecell[l]{68\%\\($r = 1.00$)}} %No redundancy
  & Random  & 46.7(39.2) & 45.7(38.4) & 42.5 \\
  & Uniform & 42.9(36.6) & 39.8(33.2) & 38.1 \\
  & IFD     & 47.0(40.3) & 33.9(27.9) & 37.2 \\
  & \textbf{\algname{}} 
             & \underline{\textbf{50.2(44.6)}} 
             & \textbf{62.5(52.1)} 
             & \underline{\textbf{52.3}} \\
\midrule
\multirow{4}{*}{\makecell[l]{51\%\\($r = 0.75$)}} 
  & Random  & 45.3(39.2) & 47.7(39.0) & 42.6 \\
  & Uniform & 35.4(31.5) & 40.6(33.4) & 35.2 \\
  & IFD     & 45.1(38.6) & 34.5(28.9) & 36.8 \\
  & \textbf{\algname{}} 
             & \textbf{48.5(43.5)} 
             & \textbf{62.7(52.7)} 
             & \textbf{51.8} \\
\midrule
\multirow{4}{*}{\makecell[l]{35\%\\($r = 0.50$)}} 
  & Random  & 45.6(39.2) & 43.7(36.9) & 41.4 \\
  & Uniform & 29.7(25.8) & 39.4(32.7) & 31.9 \\
  & IFD     & 45.5(39.2) & 33.3(27.8) & 36.5 \\
  & \textbf{\algname{}} 
             & \textbf{46.4(41.7)} 
             & \textbf{61.1(50.6)} 
             & \textbf{49.9} \\
\bottomrule
\end{tabular}}
\end{minipage}

\end{table*}


%\begin{table*}[t]
% \centering
% \caption{Performance of different data sampling strategies for \textit{CodeLlama-7B} fine-tuned on \textit{Evol-Instruct-Code-80K}. 
% The 51\% and 35\% settings correspond to 75\% and 50\% subsamples of the 68\% pruned dataset, respectively.
% Scores are pass@1 on code generation benchmarks evaluated through greedy-decoding.
% \textbf{Bold} indicates the best performance within each data-ratio setting, and \underline{underline} marks the best overall score across all configurations.}
% \label{tab:main_table}
% \begin{tabular}{l l ccccc}
% \toprule
% \textbf{Data Ratio} & \textbf{Sampling} & \textbf{HumanEval} & \textbf{HumanEval+} & \textbf{MBPP} & \textbf{MBPP+} & \textbf{Average} \\
% \midrule
% \multirow{2}{*}{100\%} 
%   & Random & 48.6 & 41.9 & \underline{64.5} & \underline{53.3} & 52.1 \\
%   & Uniform & 43.3 & 37.4 & 33.0 & 28.1 & 35.5 \\
% \midrule
% \multirow{4}{*}{\makecell[l]{68\%\\(Non-redundancy)}} 
%   & Random & 46.7 & 39.2 & 45.7 & 38.4 & 42.5 \\
%   & Uniform & 42.9 & 36.6 & 39.8 & 33.2 & 38.1 \\
%   & IFD & 47.0 & 40.3 & 33.9 & 27.9 & 37.2 \\
%   & \textbf{\algname{}}    & \underline{\textbf{50.2}} & \underline{\textbf{44.6}} & \textbf{62.5} & \textbf{52.1} & \underline{\textbf{52.3}} \\
% \midrule
% \multirow{4}{*}{\makecell[l]{51\%\\($r = 0.75$)}} 
%   & Random & 45.3 & 39.2 & 47.7 & 39.0 & 42.6 \\
%   & Uniform & 35.4 & 31.5 & 40.6 & 33.4 & 35.2 \\
%   & IFD & 45.1 & 38.6 & 34.5 & 28.9 & 36.8 \\
%   & \textbf{\algname{}}    & \textbf{48.5} & \textbf{43.5} & \textbf{62.7} & \textbf{52.7} & \textbf{51.8} \\
% \midrule
% \multirow{4}{*}{\makecell[l]{35\%\\($r = 0.50$)}} 
%   & Random & 45.6 & 39.2 & 43.7 & 36.9 & 41.4 \\
%   & Uniform & 29.7 & 25.8 & 39.4 & 32.7 & 31.9 \\
%   & IFD & 45.5 & 39.2 & 33.3 & 27.8 & 36.5 \\
%   & \textbf{\algname{}}    & \textbf{46.4} & \textbf{41.7} & \textbf{61.1} & \textbf{50.6} & \textbf{49.9} \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption[Performance of different data sampling strategies for \textit{CodeLlama-7B} fine-tuned on \textit{Evol-Instruct-Code-80K}]{Performance of different data sampling strategies for \textit{CodeLlama-7B} fine-tuned on \textit{Evol-Instruct-Code-80K}. 
% Scores are pass@1 on code generation benchmarks evaluated through greedy-decoding.}
% \label{tab:main_table}
% \begin{tabular}{l l ccccc}
% \toprule
% \textbf{Data Ratio} & \textbf{Sampling} & \textbf{HumanEval} & \textbf{HumanEval+} & \textbf{MBPP} & \textbf{MBPP+} & \textbf{Average} \\
% \midrule
% \multirow{2}{*}{100\% } 
%   & Random & 48.6 & 41.9 & 64.5 & 53.3 & 52.1 \\
%   & Uniform & 43.3 & 37.4 & 33.0 & 28.1 & 35.5 \\
% \midrule
% \multirow{3}{*}{68\%} 
%   & Random & 46.7 & 39.2 & 45.7 & 38.4 & 42.5 \\
%   & Uniform & 42.9 & 36.6 & 39.8 & 33.2 & 38.1 \\
%   & \textbf{OURS}    & \textbf{47.2} & \textbf{42.9} & \textbf{62.7} & \textbf{53.1} & \textbf{51.5} \\
% \midrule
% \multirow{3}{*}{51\%} 
%   & Random & 45.3 & 39.2 & 47.7 & 39.0 & 42.6 \\
%   & Uniform & 35.4 & 31.5 & 40.6 & 33.4 & 35.2 \\
%   & \textbf{OURS}    & \textbf{47.6} & \textbf{42.7} & \textbf{61.4} & \textbf{50.5} & \textbf{50.5} \\
% \midrule
% \multirow{3}{*}{35\%} 
%   & Random & 45.6 & 39.2 & 43.7 & 36.9 & 41.4 \\
%   & Uniform & 29.7 & 25.8 & 39.4 & 32.7 & 31.9 \\
%   & \textbf{OURS}    & \textbf{46.6} & \textbf{41.1} & \textbf{61.8} & \textbf{50.8} & \textbf{50.1} \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> table_optimization.tex <==

\begin{table}[t]
\centering
\caption{
Average gradient diversity and inter-worker gradient cosine similarity of Random and \algname{}.
}
\label{tab:optimization_diagnostics}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Selection Ratio} & \textbf{Gradient Diversity $\uparrow$} & \textbf{Inter-Worker Similarity $\downarrow$} \\
\midrule
Random & 1.00 & 0.689 & 0.260 \\
\algname{} & 1.00 & \textbf{0.741} & \textbf{0.207} \\
\bottomrule
\end{tabular}
}
% \vspace{-0.1cm}
\end{table}

